Comparing Morse Complexes Using Optimal Transport: An Experimental Study

Morse complexes and Morse-Smale complexes are topological descriptors popular in topology-based visualization. Comparing these complexes plays an important role in their applications in feature correspondences, feature tracking, symmetry detection, and uncertainty visualization. Leveraging recent advances in optimal transport, we apply a class of optimal transport distances to the comparative analysis of Morse complexes. Contrasting with existing comparative measures, such distances are easy and efficient to compute, and naturally provide structural matching between Morse complexes. We perform an experimental study involving scientific simulation datasets and discuss the effectiveness of these distances as comparative measures for Morse complexes. We also provide an initial guideline for choosing the optimal transport distances under various data assumptions.

==> sec-time-varying.tex <==
\section{Time-Varying Datasets: Feature Tracking}
\label{sec:time-varying}

In this section, we check the color transfer results across multiple time steps for three datasets: {\WD}, {\HC}, and {\NS}. 
Based on the observation from previous sections, we focus on analyzing the color transfer results using FGW distance and pFGW distance, as they provide high-quality color transfer. 
$m$ is equal for all pFGW distances within each dataset.

\para{{\WD} dataset.}
\cref{fig:wind-time-varying} shows the color transfer results for consecutive time steps. 
Results using FGW distance show robustness in node coupling: although the graph structure varies, the relatively stable features have consistent colors across time steps, such as the outbound of the Morse graph, the bottom cells enclosed by cyan, blue, and purple nodes, etc. Such robust color transfer indicates implicit feature matching and tracking in the Morse graph setting.
On the other hand, results using pFGW distance keep track of commonly shared features across time steps and ignore nodes and features missing from the reference graph. 
These results help us identify the shared topological structures of the scalar field across multiple time steps.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.98\columnwidth]{figsdraft/WD-timevarying.png}
    \vspace{-2mm}
    \caption{The color transfer results for the {\WD} dataset for time step 2 to 7, using FGW and pFGW distances.}
    \label{fig:wind-time-varying}
    \vspace{-2mm}
\end{figure} 

\para{{\HC} dataset.}
For the {\HC} dataset, we consider a time gap of around 10 for time-varying scalar field analysis, as the topology variation between adjacent time steps is small.
As shown in~\cref{fig:heatedcylinder-time-varying} (middle), FGW distance successfully matches similar features between the reference and the target graph. However, the coupling using the pFGW distance fails to identify an area in the target graphs with clear differences from the reference. We suspect that because all variations happen within a small local region, the difference is hard to be reflected when we compute the distance between two global Morse graphs.
Overall, we observe nice correspondence of features across time steps for this dataset.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.98\columnwidth]{figsdraft/HC-timevarying.png}
    \vspace{-2mm}
    \caption{The color transfer results for the {\HC} dataset for time step 809 to 899 at a gap of 10, using FGW and pFGW distances.}
    \label{fig:heatedcylinder-time-varying}
    \vspace{-2mm}
\end{figure} 

\para{{\NS} dataset.}
Following \cref{fig:navierstokes-time-varying}, we see that even with drastic changes in the Morse graph, FGW distance can conduct reasonable matchings between features. However, because we directly compare the Morse graph at $T=60$ with later time steps, the algorithm cannot notice the fact that all cell features move to the right rapidly as time goes on but keep matching the right-most feature between two Morse graphs to each other. 
Meanwhile, from the results using pFGW distance, we see the coupling ignores the additional loop features in the Morse graph at $T=63$, but it also ignores nodes that can be reasonably matched in $T=61, 63, 64$. Since we enforce a unified $m$ value in the dataset, it is hard to guarantee that only noises are ignored in the correspondence, given that the amount of noises embeded in each Morse graph is different.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.98\columnwidth]{figsdraft/NS-timevarying.png}
    \vspace{-2mm}
    \caption{The color transfer results for the {\NS} dataset for time step 60 to 66, using FGW and pFGW distances.}
    \label{fig:navierstokes-time-varying}
    \vspace{-2mm}
\end{figure} 
